RAW-Adapter: Adapting Pre-trained Visual Model to Camera RAW Images and A Benchmark

In the computer vision community, the preference for pre-training visual models has largely shifted toward sRGB images due to their ease of acquisition and compact storage. However, camera RAW images preserve abundant physical details across diverse real-world scenarios. Despite this, most existing visual perception methods that utilize RAW data directly integrate image signal processing (ISP) stages with subsequent network modules, often overlooking potential synergies at the model level. Building on recent advances in adapter-based methodologies in both NLP and computer vision, we propose RAW-Adapter, a novel framework that incorporates learnable ISP modules as input-level adapters to adjust RAW inputs. At the same time, it employs model-level adapters to seamlessly bridge ISP processing with high-level downstream architectures. Moreover, RAW-Adapter serves as a general framework applicable to various computer vision frameworks. Furthermore, we introduce RAW-Bench, which incorporates 17 types of RAW-based common corruptions, including lightness degradations, weather effects, blurriness, camera imaging degradations, and variations in camera color response. Using this benchmark, we systematically compare the performance of RAW-Adapter with state-of-the-art (SOTA) ISP methods and other RAW-based high-level vision algorithms. Additionally, we propose a RAW-based data augmentation strategy to further enhance RAW-Adapter's performance and improve its out-of-domain (OOD) generalization ability. Extensive experiments substantiate the effectiveness and efficiency of RAW-Adapter, highlighting its robust performance across diverse scenarios.

==> main/1-intro_old.tex <==
\section{Introduction}
\label{sec1:intro}


\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{pics/Motivation.pdf}
    \caption{Performance of RAW-based visual tasks with and without sRGB pre-trained weights. We analyze two methods: Dirty-Pixel~\cite{steven:dirtypixels2021} and RAW-Adapter. Blue line represents trained with MS COCO~\cite{COCO_dataset} pre-train weights, the green line indicates ImageNet~\cite{imagenet_cvpr09} pre-train weights, and the red line signifies training from scratch. We separately present the detection performance on the PASCAL RAW~\cite{omid2014pascalraw} and LOD~\cite{LOD_BMVC2021} datasets.}
    \label{fig:pretrain_weights}
    \vspace{-5mm}
\end{figure}

\IEEEPARstart{I}{n} recent years, there has been a growing interest in revisiting vision tasks using  unprocessed camera RAW images. How to leverage information-rich RAW image in computer vision tasks has become a current research hotspot in various sub-areas (\textit{i.e.} denoising~\cite{brooks2019unprocessing,zamir2020cycleisp}, view synthesis~\cite{RAW_NeRF,jin2024le3d}, object detection~\cite{Hardware_in_the_loop,LOD_BMVC2021}). Compared to commonly used sRGB image, the RAW image directly acquired by the camera sensor, encompasses abundant information unaffected or compressed by the image signal processor (ISP), and also offers physically meaningful information such as noise distributions~\cite{Dancing_under_light,Wei_2020_CVPR}, due to its linear correlation between image intensity and the radiant energy received by a camera. The acquisition of RAW data, which facilitates enhanced detail capture and a higher dynamic range, imparts a unique advantage in addressing visual tasks under variable lighting conditions in the real world. For example, sunlight irradiance can reach as high as $1.3 \times 10^3 W/m^2$, while bright planet irradiance can reach as low as $2.0 \times 10^{-6} W/m^2$~\cite{Siggraph_Physic_night_sky}.

 Meanwhile, sRGB has emerged as the primary choice for pre-training visual models in today's computer vision field, due to its scalability and ease of storage. Typically, sRGB images are derived from camera RAW data through the ISP pipeline. As shown in Fig.~\ref{fig:motivation}(a), the entire ISP pipeline consists of multiple modules to convert RAW images into human vision-oriented sRGB images, each of these modules serves its own distinct purpose, the majority being ill-posed and heavily dependent on prior information~\cite{ISP_2005,Michael_eccv16,heide2014flexisp,Camera_Net,Mobile_Computational,Joint_denoising_demosaicing}. 
 When using camera RAW data for computer vision tasks, the purpose of a manually designed ISP is to produce images that offer a superior visual experience~\cite{Vision_ISP_ICIP,steven:dirtypixels2021}, rather than optimizing for downstream visual tasks such as object detection or semantic segmentation (see  Fig.~\ref{fig:motivation}(b)). Also most manufacturers' ISPs are black boxes, making it difficult to obtain information about the specific steps inside. Consequently, utilizing a human vision oriented  ISP to process RAW data for visual tasks in downstream networks may not always yield optimal results, and in certain conditions would be less satisfactory than working directly with RAW data \cite{Bayer_RAW_HOG,LOD_BMVC2021}.


To better take advantage of camera RAW data for various computer vision tasks. Researchers began to optimize the image signal processor (ISP) jointly with downstream networks. Since most ISP stages are non-differentiable and cannot be jointly backpropagation, there are two main lines of approaches to connect ISP stages with downstream networks (see Fig.~\ref{fig:motivation}(c)): \ding{172}. First-kind approaches maintain the modular design of the traditional ISP, involving the design of differentiable ISP modules through optimization algorithms~\cite{Hardware_in_the_loop,Vision_ISP_ICIP,yu2021reconfigisp}, such as Hardware-in-the-loop~\cite{Hardware_in_the_loop} adopt covariance matrix adaptation evolution strategy (CMA-ES)~\cite{CMA-ES}. \ding{173}. Second-kind approaches replaced the ISP part entirely with a neural network~\cite{Attention_ISP_ECCV,steven:dirtypixels2021,DynamicISP_2023_ICCV,RAW_OD_CVPR2023}, such as Dirty-Pixel~\cite{steven:dirtypixels2021} adopt a stack of residual UNets~\cite{UNet} as pre-encoder, however, the additional neural network introduces a significant computational burden, especially when dealing with high-resolution inputs. 
Beyond these, the above-mentioned methods still treat ISP and the backend neural network as two independent modules, lacking interaction capabilities between two separate models. Especially, current visual models predominantly pre-trained on large amounts of sRGB images, 
there exists a significant gap between pre-trained models and camera RAW images. As shown in Fig.~\ref{fig:pretrain_weights}, training from scratch with RAW data can significantly impair the performance of RAW-based vision tasks. Leveraging sRGB pre-trained weights has proven to be highly beneficial for camera RAW-based vision tasks. Hence, we ask: Is there a more effective way to adapt \textbf{information-rich} RAW data to \textbf{knowledge-rich} sRGB pre-trained models?

\begin{figure*}
    \centering
    \includegraphics[width=1.00\linewidth]{pics/Fig1.pdf}
    
    \caption{(a). An overview of basic image signal processor (ISP) pipeline. (The sequence or configuration may vary depending on the specific ISP settings of different manufacturers.) (b). ISP and current high-level vision models have different objectives. (c) Previous methods optimize ISP with down-stream high-level vision models. (d) Our proposed RAW-Adapter.}
    \label{fig:motivation}
    \vspace{-3mm}
\end{figure*}


Our solution, RAW-Adapter, different like previous approaches that employed complex ISP or deeper neural networks at the input level. Instead, we prioritize simplifying the input stages and enhancing integration between the ISP and subsequent networks at the model level. Inspired by recent advancements in prompt learning and adapter tuning~\cite{Prompt_NLP,VPT_ECCV2022,Vit_adapter,potlapalli2023promptir}, we developed two novel adapter approaches aimed at enhancing the integration between RAW input and sRGB pre-trained models. Leveraging priors from ISP stages, our method includes input-level adapters and model-level adapters, as illustrated in Fig.~\ref{fig:motivation}(d). Input-level adapters are designed to adapt the input from RAW data to the backend network input, we follow traditional ISP design and predict ISP stages' key parameters to accommodate RAW image into the specific down-stream vision tasks, in this part, we employ strategies involving Query Adaptive Learning (QAL) and Implicit Neural Representation (INR) to ensure the differentiability of the core ISP processes while also upholding a lightweight design. Model-level adapters leverage prior knowledge from the input-level adapters by extracting intermediate stages as features, these features are then embedded into the downstream network, thus the network incorporates prior knowledge from the ISP stages, then jointly contributes to final machine-vision perception tasks.

There are still two key challenges in camera RAW-based vision tasks. The first is that current visual models are predominantly pre-trained on large datasets of sRGB images (e.g., MS-COCO~\cite{COCO_dataset}, ImageNet~\cite{imagenet_cvpr09}), creating a significant gap between pre-trained models and camera RAW images. As shown in Fig.~\ref{}, training from scratch with RAW data can severely degrade performance in RAW-based vision tasks. The second challenge is the scarcity of RAW image data, which limits the applicability of RAW-based vision tasks in diverse real-world scenarios. This is particularly problematic when training and testing conditions differ, such as varying lighting, atmospheric conditions, and different image sensor color responses. Ensuring that trained models can generalize across these varied real-world conditions remains a significant hurdle.



Our contribution in this work could be summarized as follow:

==> main/edit.tex <==
\begin{table*}[]
\caption{Comparison results (mAP $\%$) on PASCAL RAW-D dataset, we evaluate performance under normal condition and 15 different degradations ($\bigstar$: lightness corruption, $\clubsuit$: weather corruption, $\spadesuit$: blurry, $\blacksquare$: camera imaging degradation). Red background color shows
best mAP result meanwhile yellow shows second best mAP result.}
\label{tab:PASCAL-RAW}
\renewcommand\arraystretch{1.3}
\Large
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|ccccccccc}
\toprule \toprule
\multirow{2}{*}{\colorbox{red!30}{Conditions}}    & \multicolumn{9}{c}{RetinaNet~\cite{lin2017focal_loss} \colorbox{yellow!30}{with} ResNet18 (ResNet50) backbone}                                             \\ \cline{2-10} 
                     & RAW & log-RGB~\cite{log-RGB} & colorimetric~\cite{Colorimetric} & Kar.~\colorbox{yellow!30}{et al.}~\cite{Michael_eccv16} & Lite-ISP~\cite{RAW-to-sRGB_ICCV2021} & InvISP~\cite{invertible_ISP} & Dirty-Pixel~\cite{steven:dirtypixels2021} & Reconfig-ISP~\cite{yu2021reconfigisp} & \colorbox{red!30}{RAW-Adapter} \\ \hline
Normal     &  87.7 (89.2) & \colorbox{red!30}{88.9} (\colorbox{yellow!30}{89.5})  & 87.7 (89.0) & 86.0 (89.4) &  85.2 (89.3) &  84.1 (89.1) & 88.6 (89.0)  &  88.3 (89.4)   &  \colorbox{yellow!30}{88.7} (\colorbox{red!30}{89.6})     \\ \hline
Low-light $\bigstar$  & 80.3 (82.6) & 80.6 (82.3)  & 80.4 (80.9)  &  \colorbox{yellow!30}{81.9} (\colorbox{yellow!30}{84.6})  &    71.9 (73.5)    & 70.9 (74.7)  & 80.8 (83.6)  &  81.5 (83.8)   & \colorbox{red!30}{82.5} (\colorbox{red!30}{86.6})    \\ \hline
Overexposure $\bigstar$ & 87.7 (88.8) & 88.0 (89.1) &  87.4 (88.6)  & 85.6 (86.8)  & 84.2 (85.1) & 86.6 (87.3) & 88.0 (89.0) & \colorbox{yellow!30}{88.2} (\colorbox{yellow!30}{89.1}) &  \colorbox{red!30}{88.7} (\colorbox{red!30}{89.4}) \\ \hline
Flare $\bigstar$ & 84.0 (87.0) & 84.5 (85.2) & 84.2 (86.5)  & 76.4 (77.3) & 80.1 (80.8) & 82.9 (86.9)   &  \colorbox{yellow!30}{85.5} (\colorbox{red!30}{88.9})   & \colorbox{red!30}{85.6} (87.0) & \colorbox{yellow!30}{85.5} (\colorbox{yellow!30}{88.2}) \\ \hline
Low $\&$ Flare $\clubsuit$  & \colorbox{yellow!30}{64.3} (\colorbox{yellow!30}{68.5}) &  64.0 (67.3) &  62.9 (65.6) &  54.8 (58.2) & 58.8 (64.2) & 62.3 (67.9) & \colorbox{red!30}{65.1} (\colorbox{red!30}{69.6}) & 63.2 (65.9) & \colorbox{yellow!30}{64.3} (66.2)  \\ \hline
Fog $\clubsuit$  & 78.5 (79.4) & 78.7 (79.0)  & 78.6 (78.8) &  76.7 (76.8) & 75.6 (74.4) & 78.7 (79.3) &  76.9 (78.0)  & \colorbox{yellow!30}{80.3} (\colorbox{yellow!30}{79.6}) & \colorbox{red!30}{80.5} (\colorbox{red!30}{81.4})   \\ \hline
Rain $\clubsuit$ & 83.6 (86.0)  & 83.9 (85.9) & 83.8 (86.3) &  78.7 (80.1) & 79.0 (80.0)  &  83.9 (\colorbox{red!30}{86.6})  & \colorbox{yellow!30}{84.0} (84.9) & 82.9 (86.3) &  \colorbox{red!30}{84.2} (\colorbox{red!30}{86.9})  \\ \hline
Rain \& Fog $\clubsuit$   & 80.8 (\colorbox{yellow!30}{81.3}) & 80.7 (81.0) & 80.8 (81.0) & 73.5 (74.3) &  79.9 (80.0) & 80.5 (81.2) &  \colorbox{yellow!30}{81.0} (\colorbox{red!30}{81.4}) & 78.5 (80.9) &     \colorbox{red!30}{81.1} (\colorbox{red!30}{81.4})  \\ \hline
Snow $\clubsuit$  & 78.7 (80.5) & \colorbox{yellow!30}{79.5} (80.9) & 79.3 (80.3) & \colorbox{red!30}{80.3} (\colorbox{red!30}{81.3})  &  78.6 (80.5) &  76.4 (80.6)   &  79.0 (\colorbox{yellow!30}{81.1})  & 78.0 (80.7) & \colorbox{yellow!30}{79.5} (80.9)  \\ \hline
Motion Blur $\spadesuit$  & 82.0 (84.7)  & 81.2 (83.9) & \colorbox{yellow!30}{82.1} (84.1) & 81.0 (83.5) &  80.8 (82.7)  & 79.8 (83.3) &  80.7 (85.3) & 82.0 (\colorbox{yellow!30}{85.9}) &  \colorbox{red!30}{82.4} (\colorbox{red!30}{86.4}) \\ \hline
Defocus Blur $\spadesuit$ & \colorbox{yellow!30}{74.5} (79.1)  &  74.2 (78.9) &  73.5 (\colorbox{yellow!30}{79.2})  &  74.0 (76.9) & 72.5 (78.0) & 73.5 (77.5) & 74.3 (78.4) & 73.8 (78.8) &  \colorbox{red!30}{74.6} (\colorbox{red!30}{79.8})  \\ \hline
Sensor Noise $\blacksquare$  & 86.2 (88.0) & 86.2 (87.9) & 86.0 (87.5) & 86.3 (87.9) & 85.8 (87.8) &  85.5 (87.8) & \colorbox{yellow!30}{86.5} (88.4) & \colorbox{red!30}{86.8} (\colorbox{yellow!30}{88.8}) & \colorbox{red!30}{86.8} (\colorbox{red!30}{88.9})    \\ \hline
CMOS Deg $\blacksquare$ & 85.0 (87.1) &  84.8 (87.1) & 85.3 (87.5) & 85.6 (87.5) & 80.3 (84.8) & 84.2 (86.9) & \colorbox{red!30}{86.1} (87.3) & 85.7 (\colorbox{yellow!30}{88.0}) &  \colorbox{yellow!30}{85.9} (\colorbox{red!30}{89.2}) \\ \hline
Vignetting $\blacksquare$ &  85.8 (86.4) &  85.8 (86.2) &   86.4 (86.8) & \colorbox{yellow!30}{87.0} (\colorbox{yellow!30}{88.1}) & 85.1 (85.4)  & 84.3 (86.0) & 86.8 (87.5) & 86.6 (87.8) & \colorbox{red!30}{88.4} (\colorbox{red!30}{89.3}) \\ \hline
Moiré Effect $\blacksquare$ & 85.0 (87.3) &  84.8 (87.0) & 85.2 (86.8) & 83.8 (84.5)  &  83.9 (84.3) &  84.7 (84.8) & 85.5 (\colorbox{yellow!30}{88.7}) & \colorbox{yellow!30}{85.9} (88.3) & \colorbox{red!30}{86.4} (\colorbox{red!30}{88.8}) \\ \hline
CA $\blacksquare$ & \colorbox{yellow!30}{81.9} (84.8) & 81.8 (84.2) & 80.9 (83.7) &  79.5 (84.2) &  77.9 (83.5)  & 76.4 (83.7) &   81.8 (84.9) & \colorbox{red!30}{84.4} (\colorbox{red!30}{85.0}) & \colorbox{red!30}{84.4} (\colorbox{red!30}{85.6}) \\ 
 \bottomrule \bottomrule
\end{tabular}
}
\vspace{-4mm}
\end{table*}

==> main/tables.tex <==
\begin{table*}[]
\caption{Comparison results (mAP $\%$) on PASCAL RAW-D dataset, we evaluate performance under normal condition and 15 different degradations ($\bigstar$: lightness corruption, $\clubsuit$: weather corruption, $\spadesuit$: blurry, $\blacksquare$: camera imaging degradation). Red background color shows
best mAP result meanwhile yellow shows second best mAP result.}
\label{tab:PASCAL-RAW}
\renewcommand\arraystretch{1.1}
\Large
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|ccccccccc}
\toprule \toprule
\multirow{2}{*}{Degradation Type}    & \multicolumn{9}{c}{RetinaNet~\cite{lin2017focal_loss} (ResNet18 backbone~\cite{he2016resnet})}                                             \\ \cline{2-10} 
                     & RAW & log-RGB & colorimetric & Karaimer~\textit{et al.} & Lite-ISP & InvISP & Dirty-Pixel & Reconfig-ISP & RAW-Adapter \\ \hline
Normal     &  87.7 (89.2) & \cellcolor{red!10}88.9 (89.5)  & 87.7 & 86.0 &  85.2  &  84.1 & 88.6  &  88.3   &  \cellcolor{yellow!10}88.7     \\ \hline
Low-light $\bigstar$  & 80.3 & 80.6  & 80.4 &  \cellcolor{yellow!10}81.9  &     71.9     & 70.9  & 80.8  &  81.5   & \cellcolor{red!10}82.5    \\ \hline
Overexposure $\bigstar$ & 87.7 & 88.0 &  87.4  & 85.6  & 84.2 & 86.6 & 88.0 & \cellcolor{yellow!10}88.2 &  \cellcolor{red!10}88.7     \\ \hline
Flare $\bigstar$ & 84.0 & 84.5  & 84.2  & 76.4 & 80.1  & 82.9   &  \cellcolor{yellow!10}85.5   & \cellcolor{red!10}85.6 & \cellcolor{yellow!10}85.5 \\ \hline
Low-light $\&$ Flare $\clubsuit$  & \cellcolor{yellow!10}64.3  &  64.0 &  62.9 &  54.8 & 58.8 & 62.3 & \cellcolor{red!10}65.1 & 63.2 & \cellcolor{yellow!10}64.3   \\ \hline
Fog $\clubsuit$  & 78.5 & 78.7  & 78.6  &  76.7 & 75.6 & 78.7 &  76.9  & \cellcolor{yellow!10}80.3 & \cellcolor{red!10}80.5   \\ \hline
Rain $\clubsuit$ & 83.6  & 83.9 & 83.8 &  78.7 & 79.0  &  83.9  & \cellcolor{yellow!10}84.0   & 82.9 &  \cellcolor{red!10}84.2  \\ \hline
Rain \& Fog $\clubsuit$   & 80.8 & 80.7 & 80.8  & 73.5 &  79.9  & 80.5 &  \cellcolor{yellow!10}81.0  & 78.5 &     \cellcolor{red!10}81.1     \\ \hline
Snow $\clubsuit$  & 78.7 & \cellcolor{yellow!10}79.5 & 79.3 & \cellcolor{red!10}80.3   &  78.6  &  76.4   &  79.0   & 78.0  & \cellcolor{yellow!10}79.5  \\ \hline
Motion Blur $\spadesuit$  & 82.0  & 81.2 & \cellcolor{yellow!10}82.1 &     81.0 &  80.8   & 79.8 &  80.7  & 82.0 &  \cellcolor{red!10}82.4 \\ \hline
Defocus Blur $\spadesuit$ & \cellcolor{yellow!10}74.5  &  74.2 &  73.5   &  74.0 & 72.5  & 73.5 & 74.3  & 73.8 &  \cellcolor{red!10}74.6  \\ \hline
Sensor Noise $\blacksquare$  & 86.2 & 86.2  & 86.0  & 86.3   & 85.8 &  85.5 & \cellcolor{red!10}86.9  & \cellcolor{yellow!10}86.8  & \cellcolor{yellow!10}86.8     \\ \hline
CMOS Degradation $\blacksquare$ & 85.0  &  84.8  & 85.3          & 85.6 &  80.3 & 84.2 & \cellcolor{red!10}86.1 & 85.7 &  \cellcolor{yellow!10}85.9 \\ \hline
Vignetting $\blacksquare$ &  85.8 &  85.8 &   86.4  & \cellcolor{yellow!10}87.0 & 85.1  & 84.3 & 86.8  & 86.6 & \cellcolor{red!10}88.4 \\ \hline
Moiré Effect $\blacksquare$ & 85.0 &  84.8 & 85.2   & 83.8   &  83.9 &  84.7   & 85.5  & \cellcolor{yellow!10}85.9  & \cellcolor{red!10}86.4 \\ \hline
Chromatic Aberration $\blacksquare$ & \cellcolor{yellow!10}81.9 & 81.8    &   80.9   &  79.5  &  77.9   & 76.4  &         81.8 & \cellcolor{red!10}84.4 & \cellcolor{red!10}84.4   \\ \midrule \midrule
\multirow{2}{*}{Degradation Type}    & \multicolumn{9}{c}{RetinaNet~\cite{lin2017focal_loss} (ResNet50 backbone~\cite{he2016resnet})}                                             \\ \cline{2-10} 
                     & RAW & log-RGB & colorimetric & Karaimer~\textit{et al.} & Lite-ISP & InvISP & Dirty-Pixel & Reconfig-ISP & RAW-Adapter \\ \hline
Normal  &  89.2  &   \cellcolor{yellow!10}89.5  &   89.0   &  89.4  &  89.3 & 89.1 &  89.0  &  89.4  & \cellcolor{red!10}89.6  \\ \hline
Low-light $\bigstar$ & 82.6 &  82.3  &  80.9 &  \cellcolor{yellow!10}84.6 &  73.5   &  74.7  & 83.6  & 83.8 &  \cellcolor{red!10}86.6  \\ \hline
Overexposure $\bigstar$ & 88.8 & \cellcolor{yellow!10}89.1   & 88.6 &  86.8   &  85.1 & 87.3 &   89.0 & \cellcolor{yellow!10}89.1 &  \cellcolor{red!10}89.4  \\ \hline
Flare $\bigstar$ & 87.0 & 84.2 &  86.5 & 77.3  & 80.8 &  86.9 &    \cellcolor{red!10}88.9 &   87.0  &  \cellcolor{yellow!10}88.2  \\ \hline
Low-light \& Flare $\bigstar$  & \cellcolor{yellow!10}68.5 &  67.3  &  65.6   &  58.2  & 64.2 & 67.9 & \cellcolor{red!10}69.6  & 65.9  & 66.2  \\ \hline
Fog  $\clubsuit$ & 75.4 & 76.0 & 75.8  &  73.8 & 74.4 &  76.3  &   78.0  & \cellcolor{yellow!10}79.6  & \cellcolor{red!10}81.4    \\ \hline
Rain  $\clubsuit$ & 86.0 & 85.9  & 86.3 & 80.1  & 80.0 & \cellcolor{yellow!10}86.6  &  84.9  & 86.3  &  \cellcolor{red!10}86.9   \\ \hline
Rain \& Fog $\clubsuit$  & 81.3 & 81.3  & 81.0             &         74.3 &  78.7  &  81.2  &  \cellcolor{red!10}81.5   & 80.9 & \cellcolor{yellow!10}81.4 \\ \hline
Snow $\clubsuit$ & 80.5 &  80.9 & 80.3  & \cellcolor{red!10}81.3 & 80.5 & 80.6 &   \cellcolor{yellow!10}81.1  & 80.7 & 80.9        \\ \hline
Motion Blur $\spadesuit$ & 84.7 & 83.9 &  84.1    &   83.5 &  82.7  & 83.3 & 85.3 & \cellcolor{yellow!10}85.9  &  \cellcolor{red!10}86.4  \\ \hline
Defocus Blur $\spadesuit$ & 79.1 &  78.9 &   \cellcolor{yellow!10}79.2     &  76.9 &   78.0  & 77.5  & 78.4 & 78.8 &  \cellcolor{red!10}79.8 \\ \hline
Sensor Noise $\blacksquare$ & 88.0  &  87.9  &  87.5       &  87.9 &  87.8   &  87.8  &  88.4  & \cellcolor{yellow!10}88.8  & \cellcolor{red!10}88.9       \\ \hline
CMOS Degradation $\blacksquare$  & 87.1 &  87.1  &    87.5 & 87.5 &  84.8 & 86.9 & 87.3 & \cellcolor{yellow!10}88.0 & \cellcolor{red!10}89.2   \\ \hline
Vignetting $\blacksquare$ & 86.4 &  86.2  &  86.8   &  \cellcolor{yellow!10}88.1        &  85.4  & 86.0 &  87.5 & 87.8 & \cellcolor{red!10}89.3 \\ \hline
Moiré Effect $\blacksquare$ & 87.3 & 87.0 &  86.8   & 84.5 &  84.3  & 84.5 &   \cellcolor{yellow!10}88.7  &  88.3 & \cellcolor{red!10}88.8      \\ \hline
Chromatic Aberration $\blacksquare$ & 84.8 & 84.2 &   83.7  & 84.2 &   83.5 & 83.7 & 84.9      & \cellcolor{yellow!10}85.0 & \cellcolor{red!10}85.6 \\ \bottomrule \bottomrule
\end{tabular}
}
\vspace{-4mm}
\end{table*}

\begin{table*}[]
\caption{Comparison results (mIOU $\%$) on  iPhone XS Max-D dataset, we evaluate performance under normal condition and 15 different degradations ($\bigstar$: lightness corruption, $\clubsuit$: weather corruption, $\spadesuit$: blurry, $\blacksquare$: camera imaging degradation). Red background color shows
best mIOU result meanwhile yellow shows second best mIOU result.}
\label{tab:iPhoneXS}
\renewcommand\arraystretch{1.35}
\Large
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|ccccccccc}
\toprule \toprule
\multirow{2}{*}{\textbf{Conditions}}    & \multicolumn{9}{c}{SegFormer~\cite{xie2021segformer} (MIT-B0 backbone~\cite{xie2021segformer})}                                             \\ \cline{2-10} 
                     & RAW & log-RGB~\cite{log-RGB} & colorimetric~\cite{Colorimetric} & Kar.~\textit{et al.}~\cite{Michael_eccv16} & Lite-ISP~\cite{RAW-to-sRGB_ICCV2021} & InvISP~\cite{invertible_ISP} & Dirty-Pixel~\cite{steven:dirtypixels2021} & Reconfig-ISP~\cite{yu2021reconfigisp} & \textbf{RAW-Adapter} \\ \hline
Normal & 57.55 (60.10) & \cellcolor{yellow!15}57.60 (60.24) & 57.54 (60.17) & 56.89 (60.17) & 57.31 (59.94) & 57.52 (60.12)  & \cellcolor{yellow!15}57.60 (60.54) & 57.58 (60.55) & \cellcolor{red!10}57.64 (60.70) \\ \hline
Low-light $\bigstar$  & 51.29 (57.34) & 52.23 (57.77) & 51.88 (56.52) &  50.73 (53.42) &  45.85 (50.91) & 40.36 (48.48) & 52.22 (57.45) & \cellcolor{yellow!15}52.33 (57.78) & \cellcolor{red!10}52.35 
(58.69) \\ \hline
Overexposure $\bigstar$ & 58.26 (65.90) & 56.82 (63.43) & 56.73 (63.12) &  57.65 (65.44) & 55.08 (62.82) & 54.69 (62.01) & 57.67 (66.34) & \cellcolor{yellow!15}58.29 (65.30) & \cellcolor{red!10}58.58 (66.78) \\ \hline
Flare $\bigstar$ & 55.81 (63.76) & 51.93 (63.55) & 52.08 (63.51) & 51.59 (63.01) & 53.26 (63.21) & 51.94 (63.02) & 55.13 (63.36) & \cellcolor{yellow!15}55.99 (63.02) & \cellcolor{red!10}56.33 (63.88) \\ \hline
Low \& Flare $\bigstar$  & 47.14 (53.42) & 40.18 (47.71) & 40.23 (47.73) & 38.43 (50.92) & 39.77 (44.31) & 38.84 (46.89) &  47.23 (53.21) &  \cellcolor{yellow!15}47.40 (52.80)  &  \cellcolor{red!10}47.51 (53.47) \\ \hline
Fog $\clubsuit$  & \cellcolor{yellow!15}55.65 (57.29) & 54.49 (58.11) & 53.27 (56.89) &  52.15 (59.24) & 48.94 (56.43) & 53.37 (56.72) & 55.37 (62.26) & 55.48 (60.37) & \cellcolor{red!10}55.66  (60.92) \\ \hline
Rain $\clubsuit$ & 51.88 (60.44) & 46.12 (55.21) & 46.03 (53.12) & 44.14 (53.85) & 42.91 (52.94) & 49.61 (57.33) &  51.26 (60.35) & \cellcolor{yellow!15}53.29 (60.32) &  \cellcolor{red!10}53.38 (61.86) \\ \hline
Rain \& Fog $\clubsuit$   & 51.05 (58.43) & 48.77 (56.82) &  48.03 (56.34) & 46.35 (57.75) &  44.72 (55.01) & 51.31 (54.33) &  \cellcolor{yellow!15}51.39 (58.08) & 51.33 (58.09) &  \cellcolor{red!10}51.41 (58.21)  \\ \hline
Snow $\clubsuit$  & 50.58 (57.83) & 50.65 (56.95)  & 50.54 (56.99) & 47.71 (58.32) & 46.64 (54.83) & 49.06 (55.21) & \cellcolor{yellow!15}50.71 (58.40) & 50.66 (58.12) & \cellcolor{red!10}50.94 (58.51) \\ \hline
Motion Blur $\spadesuit$  & 56.06 (63.00) & 55.44 (62.73) & 54.93 (62.62) & 54.92 (61.99) & 49.38 (60.23)  & 48.25 (61.80) & 56.22 (63.50) & \cellcolor{yellow!15}56.30 (62.44) & \cellcolor{red!10}56.49 (63.60)  \\ \hline
Defocus Blur $\spadesuit$ & 52.31 (59.03) &  52.52 (58.71) &  52.33 (58.97) & 51.57 (55.36) & 45.01 (56.24) & 44.70 (53.31) &  \cellcolor{red!10}52.74 (59.55) & \cellcolor{yellow!15}52.60 (59.00) & 52.35 (59.09) \\ \hline
Sensor Noise $\blacksquare$  & 50.46 (58.93) &  \cellcolor{yellow!15}52.16 (59.20) &  50.83 (58.87)   & 51.92 (55.92) &  50.88 (56.31) &   49.08 (53.41) &  51.25 (59.19) & 51.87 (59.20) &  \cellcolor{red!10}52.65 (59.34) \\ \hline
CMOS Deg $\blacksquare$ & 56.09 (64.29)  & 55.81 (63.21) &  54.73 (62.09) & 50.07 (61.33) & 53.21 (63.86) & 50.20 (61.29) & 56.88 (64.16)  & \cellcolor{yellow!15}56.98 (64.08) & \cellcolor{red!10}58.10 (64.46) \\ \hline
Vignetting $\blacksquare$ & \cellcolor{red!10}58.31 (66.01) & 56.87 (64.39) &  56.19 (64.52) & 56.02 (63.87) & 47.22 (63.41) & 49.18 (63.22) & 57.77 (65.84) & \cellcolor{yellow!15}58.01 (65.27) &  57.82 (65.55) \\ \hline
Moiré Effect $\blacksquare$ & 53.19 (63.35) &  52.84 (63.55) & 52.91 (63.04) & 54.21 (61.87) & 46.87 (61.52) & 44.81 (60.97) & \cellcolor{yellow!15}54.55 (63.24) & 54.38 (63.02) & \cellcolor{red!10}55.01 (63.63) \\ \hline
CA $\blacksquare$ & 53.18 (62.26) & 53.51 (62.22) & 53.28 (62.24) & 53.48 (61.81) & 46.81 (59.88) & 47.72 (60.93) &  53.35 (61.93) & \cellcolor{yellow!15}53.68 (62.22) & \cellcolor{red!10}53.76 (62.39) \\ \midrule \midrule
\multirow{2}{*}{Degradation Type}    & \multicolumn{9}{c}{SegFormer~\cite{xie2021segformer} (MIT-B3 backbone~\cite{xie2021segformer})}                                             \\ \cline{2-10} 
                     & RAW & log-RGB & colorimetric & Karaimer~\textit{et al.} & Lite-ISP & InvISP & Dirty-Pixel & Reconfig-ISP & RAW-Adapter \\ \hline
Normal  & 60.10 & 60.24 & 60.17 & 60.17 & 59.94 & 60.12 & 60.54 & \cellcolor{yellow!15}60.55 & \cellcolor{red!10}60.70 \\ \hline
Low-light $\bigstar$ & 57.34 &  57.77  &    56.52  &  53.42 & 50.91  & 48.48 & 57.45  & \cellcolor{yellow!15}57.78 & \cellcolor{red!10}58.69 \\ \hline
Overexposure $\bigstar$ & 65.90 & 63.43 & 63.12 & 65.44 & 62.82  & 62.01 & \cellcolor{yellow!15}66.34 & 65.30 & \cellcolor{red!10}66.78 \\ \hline
Flare $\bigstar$ & \cellcolor{yellow!15}63.76 & 63.55 & 63.51  & 63.01 & 63.21 & 63.02 & 63.36 & 63.02 &  \cellcolor{red!10}63.88   \\ \hline
Low-light \& Flare $\bigstar$  & \cellcolor{yellow!15}53.42 & 47.71  & 47.73 & 50.92 & 44.31 & 46.89     & 53.21 & 52.80 & \cellcolor{red!10}53.47 \\ \hline
Fog  $\clubsuit$ & 57.29 & 58.11 & 56.89 & 59.24 & 56.43 & 56.72 & \cellcolor{red!10}62.26 &  60.37 &  \cellcolor{yellow!15}60.92 \\ \hline
Rain  $\clubsuit$ & \cellcolor{yellow!15}60.44 & 55.21 &  53.12 & 53.85 & 52.94 & 57.33 & 60.35 &  60.32 & \cellcolor{red!10}61.86 \\ \hline
Rain \& Fog $\clubsuit$  & \cellcolor{red!10}58.43 & 56.82 & 56.34 & 57.75 &  55.01 & 54.33 & 58.08 & 58.09 & \cellcolor{yellow!15}58.21 \\ \hline
Snow $\clubsuit$ & 57.83 &  56.95  &   56.99  &  58.32   &  54.83  & 55.21 &   \cellcolor{yellow!15}58.40   & 58.12  & \cellcolor{red!10}58.51     \\ \hline
Motion Blur $\spadesuit$ & 63.00 &  62.73  &  62.62  &  61.99  & 60.23    & 61.80 &  \cellcolor{yellow!15}63.50 & 62.44  & \cellcolor{red!10}63.60  \\ \hline
Defocus Blur $\spadesuit$ & 59.03 &  58.71  &  58.97  & 55.36    & 56.24  & 53.31 & \cellcolor{red!10}59.55 & 59.00 & \cellcolor{yellow!15}59.09   \\ \hline
Sensor Noise $\blacksquare$ & 58.93 & \cellcolor{yellow!15}59.20  &  58.87  & 55.92  & 56.31  & 53.41  &   59.19  &  \cellcolor{yellow!15}59.20 & \cellcolor{red!10}59.34  \\ \hline
CMOS Degradation $\blacksquare$  & \cellcolor{yellow!15}64.29 & 63.21 & 62.09 &  61.33 &  63.86 & 61.29 & 64.16 & 64.08 &  \cellcolor{red!10}64.46  \\ \hline
Vignetting $\blacksquare$ & \cellcolor{red!10}66.01 &  64.39 & 64.52 &   63.87 & 63.41 & 63.22 &  \cellcolor{yellow!15}65.84 & 65.27 & 65.55 \\ \hline
Moiré Effect $\blacksquare$ & 63.35 & \cellcolor{yellow!15}63.55 & 63.04 & 61.87  &  61.52  &  60.97  &  63.24  & 63.02 & \cellcolor{red!10}63.63 \\ \hline
Chromatic Aberration $\blacksquare$ & \cellcolor{yellow!15}62.26 & 62.22       &  62.24  &  61.81  & 59.88 & 60.93 & 61.93  & 62.22 & \cellcolor{red!10}62.39  \\ \bottomrule \bottomrule
\end{tabular}
}
\vspace{-4mm}
\end{table*}
